Teaching contact-rich tasks from visual demonstrations by constraint extraction

Contact-rich manipulation involves kinematic constraints on the task motion, typically with discrete transitions between these constraints during the task. Allowing the robot to detect and reason about these contact constraints can support robust and dynamic manipulation, but how can these contact models be efficiently learned? Purely visual observations are an attractive data source, allowing passive task demonstrations with unmodified objects. Existing approaches for vision-only learning from demonstration are effective in pick-and-place applications and planar tasks. Nevertheless, accuracy/occlusions and unobserved task dynamics can limit their robustness in contact-rich manipulation. To use visual demonstrations for contact-rich robotic tasks, we consider the demonstration of pose trajectories with transitions between holonomic kinematic constraints, first clustering the trajectories into discrete contact modes, then fitting kinematic constraints per each mode. The fit constraints are then used to (i) detect contact online with force/torque measurements and (ii) plan the robot policy with respect to the active constraint. We demonstrate the approach with real experiments, on cabling and rake tasks, showing the approach gives robust manipulation through contact transitions.

==> Teaching Contact-Rich Tasks by Visual-only Demonstrations/scraps.tex <==

\iffalse 
Motivating observations:
\begin{itemize}
\item Contact-rich manipulation involves a series of discrete changes in contact constraints as contact is made or broken. These contact conditions can be used to represent or monitor a manipulation task.
\item Force information is needed for many contact-rich manipulation tasks, especially to deal with issues like occlusion or limited visual accuracy. Demonstrations with force information require either teleoperation or an additional F/T sensor to isolate the environment forces.
\item Contact models are a data-efficient way to do monitoring and control, but require information on contact geometry such as via collision detection from meshes or simple shapes. When the robot copies the demonstrations, we will probably stay near the original demonstrations, so building a local contact model may be sufficient, removing the need for full object geometry, simplifying deployment substantially.
\item Clustering methods can be used to split a continuous demonstration into a discrete set of contact modes.
\item Visual-only observations allows a human to directly manipulate a part in the desired manner, and may be needed when teleoperation is difficult (e.g. rotations, complex force-sensitive motions).
\item Demonstrations are noisy, due to either the manipulation itself or the observation system. This can limit the ability to use demonstration for contact-rich tasks. At the same time, when objects are manipulated by humans, repeatability in object trajectories will likely arise from kinematic contact constraints, due to noise in human motor control. 
\end{itemize}
\fi 

\iffalse
\subsection{Related Work}
\begin{itemize}
\item \cite{subramani2018}: use instrumented tool to demo task, fit constraints from force/position info. But no transfer to robot? \\
\item \cite{su2018}: kinesthetic demonstration, cluster, build discrete modes and a graph between them. Use direct clustering methods, no contact models built \\
\item \cite{sidhik2021}: learn contact model (contact normal + location) from robot data, focus on low-level control for transitions, not clear how initial data collected, simple tasks (sliding on planar surface) \\
\item \cite{wang2019a}: learn a discrete-level transition model from clustering contact data, just simulation, data collected from hand-defined cartesian motions, no contact normal/dynamics \\
\item \cite{davchev2022}: Dynamic motion primitives fine-tuned by RL for contact tasks.  Data collected from teleoperation, only simulation.
\end{itemize}
\fi 


We make two distinctions in types of constraints:
\begin{enumerate}
    \item Constraints which need to be {\bf enforced} by applying a contact force, such as polishing or writing on a surface, which are more naturally expressed with $g(x)\geq0$
    \item Constraints which need to be {\bf respected} and the motion in the constraint direction $J_m(x)\dot{x} \approx 0$, and are true holonomic constraints $h(x)=0$
\end{enumerate}


%@Christian:    Can't edit lib.bib :( 

@inproceedings{blomqvist2022semi,
  title={Semi-automatic 3d object keypoint annotation and detection for the masses},
  author={Blomqvist, Kenneth and Chung, Jen Jen and Ott, Lionel and Siegwart, Roland},
  booktitle={2022 26th International Conference on Pattern Recognition (ICPR)},
  pages={3908--3914},
  year={2022},
  organization={IEEE}
}


==> scraps.tex <==

\iffalse 
Motivating observations:
\begin{itemize}
\item Contact-rich manipulation involves a series of discrete changes in contact constraints as contact is made or broken. These contact conditions can be used to represent or monitor a manipulation task.
\item Force information is needed for many contact-rich manipulation tasks, especially to deal with issues like occlusion or limited visual accuracy. Demonstrations with force information require either teleoperation or an additional F/T sensor to isolate the environment forces.
\item Contact models are a data-efficient way to do monitoring and control, but require information on contact geometry such as via collision detection from meshes or simple shapes. When the robot copies the demonstrations, we will probably stay near the original demonstrations, so building a local contact model may be sufficient, removing the need for full object geometry, simplifying deployment substantially.
\item Clustering methods can be used to split a continuous demonstration into a discrete set of contact modes.
\item Visual-only observations allows a human to directly manipulate a part in the desired manner, and may be needed when teleoperation is difficult (e.g. rotations, complex force-sensitive motions).
\item Demonstrations are noisy, due to either the manipulation itself or the observation system. This can limit the ability to use demonstration for contact-rich tasks. At the same time, when objects are manipulated by humans, repeatability in object trajectories will likely arise from kinematic contact constraints, due to noise in human motor control. 
\end{itemize}
\fi 

\iffalse
\subsection{Related Work}
\begin{itemize}
\item \cite{subramani2018}: use instrumented tool to demo task, fit constraints from force/position info. But no transfer to robot? \\
\item \cite{su2018}: kinesthetic demonstration, cluster, build discrete modes and a graph between them. Use direct clustering methods, no contact models built \\
\item \cite{sidhik2021}: learn contact model (contact normal + location) from robot data, focus on low-level control for transitions, not clear how initial data collected, simple tasks (sliding on planar surface) \\
\item \cite{wang2019a}: learn a discrete-level transition model from clustering contact data, just simulation, data collected from hand-defined cartesian motions, no contact normal/dynamics \\
\item \cite{davchev2022}: Dynamic motion primitives fine-tuned by RL for contact tasks.  Data collected from teleoperation, only simulation.
\end{itemize}
\fi 


We make two distinctions in types of constraints:
\begin{enumerate}
    \item Constraints which need to be {\bf enforced} by applying a contact force, such as polishing or writing on a surface, which are more naturally expressed with $g(x)\geq0$
    \item Constraints which need to be {\bf respected} and the motion in the constraint direction $J_m(x)\dot{x} \approx 0$, and are true holonomic constraints $h(x)=0$
\end{enumerate}


%@Christian:    Can't edit lib.bib :( 

@inproceedings{blomqvist2022semi,
  title={Semi-automatic 3d object keypoint annotation and detection for the masses},
  author={Blomqvist, Kenneth and Chung, Jen Jen and Ott, Lionel and Siegwart, Roland},
  booktitle={2022 26th International Conference on Pattern Recognition (ICPR)},
  pages={3908--3914},
  year={2022},
  organization={IEEE}
}

